Extending a system in the calculus of structures with a self-dual quantifier

We recall that SBV, a proof system developed under the methodology of deep inference, extends multiplicative linear logic with the self-dual non-commutative logical operator Seq. We introduce SBVQ that extends SBV by adding the self-dual quantifier Sdq. The system SBVQ is consistent because we prove that (the analogous of) cut elimination holds for it. Its new logical operator Sdq operationally behaves as a binder, in a way that the interplay between Seq, and Sdq can model {\beta}-reduction of linear {\lambda}-calculus inside the cut-free subsystem BVQ of SBVQ. The long term aim is to keep developing a programme whose goal is to give pure logical accounts of computational primitives under the proof-search-as-computation analogy, by means of minimal, and incremental extensions of SBV.

==> BV2-structure-equivalences-singleton.tex <==
\smalltitle{\textbf{Singleton}}%
{%do not erase
 \vlstore{
   \label{align:singleton}
     \vlsbr(\strR)
   & \sim &
     \vlsbr<\strR>
     \sim
     \vlsbr[\strR]
     \sim
     \strR
 }%\vlstore
{\setlength{\arraycolsep}{2pt}
\begin{eqnarray}
 \vlread
\end{eqnarray}}
}%do not erase

==> LLCXS-beta-reduction.tex <==
\begin{align}
\label{align:beta-rule}
\llcxA{\llcxF{\llcxX}{\llcxM}}{\llcxN} &
 \llcxBeta
 \llcxE{\llcxM}{\llcxX}{\llcxN}
& (\beta\mbox{\textrm{-reduction}})
\\
\nonumber
\llcxE{\llcxX}{\llcxX}{\llcxP}         &
 \llcxBeta
 \llcxP
& (\textit{substitution})
\\
\label{align:beta-subst-clash-free}
\llcxE{(\llcxF{\llcxY}{\llcxM})}{\llcxX}{\llcxP}   &
 \llcxBeta
 \llcxF{\llcxY}{(\llcxE{\llcxM}{\llcxX}{\llcxP})}
\\
\nonumber
\llcxE{(\llcxA{\llcxM}{\llcxN})}{\llcxX}{\llcxP}   &
 \llcxBeta
 \llcxA{\llcxM}{(\llcxE{\llcxN}{\llcxX}{\llcxP})}
 \quad
 \textrm{ if } \llcxX\in\llcxFV{\llcxN}
\\
\nonumber
\llcxE{(\llcxA{\llcxM}{\llcxN})}{\llcxX}{\llcxP}   &
 \llcxBeta
 \llcxA{\llcxE{\llcxM}{\llcxX}{\llcxP}}{\llcxN}
 \quad
 \textrm{ if } \llcxX\in\llcxFV{\llcxM}
\end{align}

==> SBV2-soundness-eval-ex-leftmost-BVTDer.tex <==
{\small
\[
\vlderivation                  {
\vlde{}{}
     {\mapLcToDi{\llcxA{I}{\llcxA{I}{I}}}
                 {\atmo}}      {
\vlde{}{}
     {\mapLcToDi{\llcxA{I}{I}}{\atmo}}       {
\vlhy{\mapLcToDi{I}{\atmo}}    }}}
\]
}



==> SBV2-soundness-eval-ex-leftmost-LT.tex <==
{\small
$
\vlderivation{
\vliin{\vlrulename{\llcxSOStrarule}}{}
      {\llcxSOSJud{\llcxA{I}{\llcxA{I}{I}}}{I}}
      { % A
		\vliin{\vlrulename{\llcxSOStrarule}}{}
		      {\llcxSOSJud{\llcxA{I}{\llcxA{I}{I}}}{\llcxA{I}{I}}}
		      { % A.1
		       \vlin{\vlrulename{\llcxSOSBrule}}{}
		            {\llcxSOSJud{\llcxA{I}{\llcxA{I}{I}}}
		                         {\llcxE{\llcxX}{\llcxX}{\llcxA{I}{I}}}}
		             {\vlhy{\llcxA{I}{\llcxA{I}{I}}
		             		\llcxBeta
		             		\llcxE{\llcxX}{\llcxX}{\llcxA{I}{I}}
		             	   }}
		      }
		      { % A.2
		       \vlin{\vlrulename{\llcxSOSBrule}}{}
		            {\llcxSOSJud{\llcxE{\llcxX}{\llcxX}{\llcxA{I}{I}}}{\llcxA{I}{I}}}
		            {\vlhy{\llcxE{\llcxX}{\llcxX}{\llcxA{I}{I}}
		                   \llcxBeta
  		                   \llcxA{I}{I}
		                  }}
		      }
      }
      { % B
		\vliin{\vlrulename{\llcxSOStrarule}}{}
		      {\llcxSOSJud{\llcxA{I}{I}}{I}}
		      { % B.1
		       \vlin{\vlrulename{\llcxSOSBrule}}{}
		            {\llcxSOSJud{\llcxA{I}{I}}{\llcxE{\llcxX}{\llcxX}{I}}}
		            {\vlhy{\llcxA{I}{I}
		                   \llcxBeta
		                   \llcxE{\llcxX}{\llcxX}{I}
		                  }}
		      }
		      { % B.2
		       \vlin{\vlrulename{\llcxSOSBrule}}{}
		            {\llcxSOSJud{\llcxE{\llcxX}{\llcxX}{I}}{I}}
		            {\vlhy{\llcxE{\llcxX}{\llcxX}{I}
		                   \llcxBeta
		                   I}}
		      }
      }
}
$}

==> SBV2-soundness-eval-ex-rightmost-BVTDer.tex <==
{\small
\[
\vlderivation                                {
\vlin{\bvtsinrule}{}
     {\mapLcToDi{\llcxA{I}
                       {\llcxA{I}{I}}}
                 {\atmo}
      \equiv
      \vlex{\atmp}
           {{\vlsmallbrackets
             \vlsbr[\mapLcToDi{I}{\atmp}
                   ;\vlex{\atmq}{\mapLcToDi{
		     \llcxA{I}{I}          }{\atmq}}
                   ;(\atmp;\natmo)]}}
     }                                      {
\vlin{\bvtsvarule}{}
     {\vlex{\atmp}
           {{\vlsmallbrackets
             \vlsbr[\mapLcToDi{I}{\atmp}
                   ;\vlex{\atmq}{\mapLcToDi{\llcxE{\llcxX}
                                                  {\llcxX}
                                                  {I}
                                           }
                                           {\atmq}
                                }
                   ;(\atmp;\natmo)]}}
     }                                               {
\vlin{\bvtsinrule}{}
     {\mapLcToDi{\llcxA{I}{I}
                }{\atmo}
      \equiv
      \vlex{\atmp}
           {{\vlsmallbrackets
             \vlsbr[\mapLcToDi{I}{\atmp}
                   ;\vlex{\atmq}{\mapLcToDi{I
                                           }
                                           {\atmq}
                                }
                   ;(\atmp;\natmo)]}}
      }                                               {
\vlin{\bvtsvarule}{}
     {\mapLcToDi{\llcxE{\llcxX}
                       {\llcxX}
                 {I}}
                 {\atmo}} {
\vlhy{\mapLcToDi{I}{\atmo}}            }}}}}
\]}
 


==> SBV2-soundness-eval-ex-rightmost-LT.tex <==
%{\small
%\[
%\infer[\!]
%{
%}
%{
%  \infer[\!]
%  {
%  }
%  {
%   \infer[\!]
%   {
%   }
%   {\infer[\!]
%    {
%    }
%    {
%    }
%    \quad
%    \infer[\!]
%    {
%    }
%    {
%    }
%   }
%  }
%  \quad
%  \infer[\!]
%  {
%  }
%  {
%    \infer[\!]
%    {
%    }
%    {
%    }
%    \quad
%    \infer[\!]
%    {\llcxSOSJud{\llcxE{\llcxX}{\llcxX}{I}}{I}
%    }
%    {
%    }
%  }
%}
%\]} 

{\small
$
\vlderivation{
\vliin{\vlrulename{\llcxSOStrarule}}{}
      {\llcxSOSJud{\llcxA{I}{\llcxA{I}{I}}}{I}}
      { %A
       \vlin{\vlrulename{\llcxSOSarrule}}{}
            {\llcxSOSJud{\llcxA{I}{\llcxA{I}{I}}}{\llcxA{I}{I}}}
            { 
             \vliin{\vlrulename{\llcxSOStrarule}}{}
                   {\llcxSOSJud{\llcxA{I}{I}}{I}}
                   { %A.1
                    \vlin{\vlrulename{\llcxSOSBetarule}}{}
                         {\llcxSOSJud{\llcxA{I}{I}}{\llcxE{\llcxX}{\llcxX}{I}}}
                         {\vlhy{}
                         }
                   } %A.1
                   { %A.2
                    \vlin{\vlrulename{\llcxSOSBetarule}}{}
                         {\llcxSOSJud{\llcxE{\llcxX}{\llcxX}{I}}
                                     {I}}
                         {\vlhy{}
                         }
                   } %A.2
            }
      } %A
      { %B
       \vliin{\vlrulename{\llcxSOStrarule}}{}
             {\llcxSOSJud{\llcxA{I}{I}}{I}}
             { %B.1 
              \vlin{\vlrulename{\llcxSOSBetarule}}{}
                   {\llcxSOSJud{\llcxA{I}{I}}{\llcxE{\llcxX}{\llcxX}{I}}}
                   {
		            \vlhy{}
                   }
             } %B.1
             { %B.2
              \vlin{\vlrulename{\llcxSOSBetarule}}{}
                   {\llcxSOSJud{\llcxE{\llcxX}{\llcxX}{I}}
                               {I}}
                   {
		            \vlhy{}
                   }
             } %B.2
      } %B
 }
$
} %\small

==> SBV2-soundness.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[\textbf{\textit{Weak Soundness of $\BVT$}}]
\label{theorem:Weak soundness of SBVT}
For every $\llcxM, \llcxN$, and $\llcxo$, let
$\bvtInfer{\bvtDder}{\mapLcToDi{\llcxN}{\atmo}
 \bvtJudGen{\BVT}{}
 \mapLcToDi{\llcxM}{\atmo}}$ be derived by a, possibly empty, sequence of
instances of $\bvtsinrule$ (Lemma~\ref{lemma:Simulating llcxBeta}.) Then
$\llcxSOSJud{\llcxM}{\llcxN}$.
\end{theorem}
\begin{proof}
By induction on $\Size{\bvtDder}$, proceeding by cases on the form of
$\llcxM$ and $\llcxN$.
(Details in Appendix~\ref{section:Proof of Weak soundness of SBVT}.)
\end{proof}
